Iterative Program Synthesis for Adaptable Social Navigation

Robot social navigation is influenced by human preferences and environment-specific scenarios such as elevators and doors, thus necessitating end-user adaptability. State-of-the-art approaches to social navigation fall into two categories: model-based social constraints and learning-based approaches. While effective, these approaches have fundamental limitations -- model-based approaches require constraint and parameter tuning to adapt to preferences and new scenarios, while learning-based approaches require reward functions, significant training data, and are hard to adapt to new social scenarios or new domains with limited demonstrations. In this work, we propose Iterative Dimension Informed Program Synthesis (IDIPS) to address these limitations by learning and adapting social navigation in the form of human-readable symbolic programs. IDIPS works by combining program synthesis, parameter optimization, predicate repair, and iterative human demonstration to learn and adapt model-free action selection policies from orders of magnitude less data than learning-based approaches. We introduce a novel predicate repair technique that can accommodate previously unseen social scenarios or preferences by growing existing policies. We present experimental results showing that IDIPS: 1) synthesizes effective policies that model user preference, 2) can adapt existing policies to changing preferences, 3) can extend policies to handle novel social scenarios such as locked doors, and 4) generates policies that can be transferred from simulation to real-world robots with minimal effort.

==> dipr_fig.tex <==
\begin{figure}[htb!]
  \vspace{-1em}
\begin{lstlisting}[language=Python, mathescape=true,
xleftmargin=0.05\textwidth,
basicstyle=\scriptsize\ttfamily,
  numbers=left, escapechar=!]
!\(\begin{array}{@{}l}
  \texttt{\textbf{Repair}} :
      \nat \times \real \times \worlds \times \worlds \times \pred
      \rightarrow \pred
\end{array}\)!
$\texttt{Repair}$($\maxDepth$, $\minScore$, $\posE$, $\negE$, $\pred$):
  $\texttt{falseNeg} = \texttt{Score}(\pred, \posE, \emptyset) \neq 1.0$
  $\texttt{falsePos} = \texttt{Score}(\pred, \negE, \emptyset) \neq 1.0$
  if ($\texttt{falsePos}$ and $\texttt{falseNeg}$): $\pred = (\pred \land \ppred) \lor (\ppred \land \ppred')$
  elif ($\texttt{falseNeg}$): $\pred = \pred \lor \ppred$
  elif ($\texttt{falsePos}$): $\pred = \pred \land \ppred$
  return $\texttt{Synthesize}(\maxDepth, \minScore, \posE \cup \negE, \pred)$
\end{lstlisting}
  \vspace{-1em}
  \caption{Predicate Repair Module}
\figlabel{dipr}
  \vspace{-1em}
\end{figure}

% !\(\begin{array}{@{}l}
  % \texttt{\textbf{Score}} :
      % \pred \times \worlds \times \worlds
      % \rightarrow \real
% \end{array}\)!
  % $\pred' = {\arg\max}_{\pred'}~\texttt{Score}(\texttt{Synthesize}(\maxDepth, \env, \posE, \negE, \pred'), \posE, \negE)$
    % $\given \pred'',\pred''' \in \texttt{EnumPredicates}(\maxDepth)$


==> dipr_synth.tex <==
\begin{figure*}[!thb]
  \begin{subfigure}{0.33\textwidth}
\begin{minipage}[htb!]{0.33\textwidth}
\begin{lstlisting}[language=Python, mathescape=true,numbers=left,
                   xleftmargin=0.5\textwidth,
                   basicstyle=\scriptsize\ttfamily, escapechar=!]
!\(\begin{array}{@{}l}
  \texttt{\textbf{ParamSynth}} :
      \worlds \times \worlds \times \pred \rightarrow \pred
\end{array}\)!
$\texttt{ParamSynth}$($\posE$, $\negE$, $\pred$):
  $\vec{?\param} = \texttt{ParamHoles}(\pred)$
  !\(\begin{array}{@{}l@{}l@{}l}
    \phi & = & \exists \vec{?\param} \\
    & \mid &
    (\forall \world \in \posE~.~\texttt{PartialEval}(\pred, \world))\land \\
    & &
    (\forall \world \in \negE~.~\neg\texttt{PartialEval}(\pred, \world))
  \end{array}\)!
  return $\texttt{Optimize}$($\phi$) #$\texttt{MaxSMT}$
!\(\begin{array}{@{}l}
  \texttt{\textbf{ParamHoles}} : \pred \rightarrow [?\param]
\end{array}\)!
!\(\begin{array}{@{}l}
    \texttt{\textbf{PartialEval}} : \pred \times \world \rightarrow \pred
\end{array}\)!
\end{lstlisting}
\end{minipage}
    \caption{Parameter Synthesis}
\figlabel{paramSynth}
  \end{subfigure}
% L2
  \begin{subfigure}{0.3\textwidth}
\begin{minipage}[htb!]{0.38\textwidth}
  \scriptsize
\begin{lstlisting}[language=Python, mathescape=true,
  xleftmargin=0.5\textwidth,
  basicstyle=\scriptsize\ttfamily, numbers=none, numbers=left, escapechar=!]
!\(\begin{array}{@{}l}
  \texttt{\textbf{ExprSynth}} :
      \nat \times \worlds \times \worlds \times \pred
      \rightarrow \pred
\end{array}\)!
$\texttt{ExprSynth}$($\posE$, $\negE$, $\pred$):
  $\exprs$ = $\texttt{EnumFeatures}$($\posE \cup \negE$) !\label{line:enumFeatures}!
  $\pred' = {\arg\max}_{\pred'}~
    \texttt{Score}($
    $\texttt{ParamSynth}(\posE, \negE, \pred'), \posE, \negE)$
      $\given \pred' \in \texttt{FillExpressions}(\exprs)$
  return $\pred'$
!\(\begin{array}{@{}l}
    \texttt{\textbf{FillExpressions}} : \exprs \times \pred \rightarrow \{\pred\}
\end{array}\)!
!\(\begin{array}{@{}l}
    \texttt{\textbf{SigFilter}} : \{ \langle \expr, \sig \rangle \} \rightarrow
                         \{ \langle \expr, \sig \rangle \}
\end{array}\)!
!\(\begin{array}{@{}l}
  \texttt{\textbf{EnumPredicates}} : \nat \rightarrow \{ \pred \}
\end{array}\)!
!\(\begin{array}{@{}l}
\texttt{\textbf{EnumFeatures}} : \nat \times \worlds \rightarrow \{ \expr \}
\end{array}\)!
\end{lstlisting}
  % \hrule
  % \vspace{3pt}
  % FillExpressions Def
  \scriptsize
% \end{minipage}
% \vrule
% \hspace{0.5em}
% \begin{minipage}[htb!]{0.45\textwidth}
  \scriptsize
  % \footnotesize
  % enum features
  % \(\begin{array}{@{}l}
    % \texttt{\textbf{EnumFeatures}} :
    % \nat \times \env \times \type \times \worlds \times \expr
    % \rightarrow \{\langle \expr, \sig \rangle\} \\
    % % \texttt{\textbf{Base Case}} \\
    % \texttt{EnumFeatures}(0, \env, \type, \worldSet, \expr) = \{~\} \\
    % % Expansion Rules for hole
    % % \texttt{\textbf{Top-Level Expansion Rule}} \\
    % \texttt{EnumFeatures}(\depth + 1, \env, \type, \worldSet, ?\expr)
    % = \texttt{SigFilter(} \\
    % % Try filling in a constant value
    % % Try filling in an input
    % \quad \{\texttt{EnumFeatures}(\depth, \env, \type, \worldSet, \expr),  \forall \expr : \type \in \env\}~\cup \\
    % % Try applying op1
    % \quad \{\texttt{EnumFeatures}(\depth + 1, \env, \type, \worldSet, \uOp{?\expr}), \\
     % \forall \uOpE : \type' \rightarrow \type \in \env\}) \\
    % % Try Applying op2
    % % \quad \{\texttt{EnumFeatures}(\depth + 1, \env, \type, \worldSet,
    % % \bOp{?\expr}{?\expr}), \\
    % % \qquad  \forall \bOpE : \type' \times \type'' \rightarrow \type \in \env\}) \\
    % % Fundamental constant case
    % % \texttt{\textbf{Fundamental Constant Expansion}} \\
    % \texttt{EnumFeatures}(\depth+1, \env, \type, \worldSet, \const) =
    % \{~\langle \const, \sig \rangle  \\
    % \quad \given \sig = [\const,\dots,\const],
    % \forall \world^i \in \worldSet \}\\
    % % Input Var Case
    % % \texttt{\textbf{Input Variable Expansion}} \\
    % \texttt{EnumFeatures}(\depth+1, \env, \type, \worldSet, \inputVar) =
    % \{~\langle \inputVar, \sig \rangle\ \\
    % \quad \given \sig = [\world^i.\inputVar,\dots,\world^n.\inputVar],
    % \forall \world^i \in \worldSet \} \\
    % % Unary Op Case
    % % \texttt{\textbf{Unary Operator Expansion}} \\
    % \texttt{EnumFeatures}(\depth+1, \env, \type, \worldSet, \uOp{\expr}) =
    % \{~\langle \uOp{\inputVar}, \sig \rangle \\
    % \quad \given \uOpE : \type' \rightarrow \type \in \env,~\sig =
    % [\interp(\uOp{\expr'},\world) \given \world \in \worldSet], \\
    % \qquad\forall \expr' \in
    % \texttt{EnumFeatures}(\depth, \env, \type', \worldSet, ?\expr) \} \\
    % % Binary Op Case
    % % \texttt{\textbf{Binary Operator Expansion}} \\
    % % \texttt{EnumFeatures}(d+1, \env, \type, \worldSet, \bOp{\expr_1}{\expr_2}) =
    % % \{~ \langle \uOp{\inputVar}, \sig \rangle\ \\
    % % \quad  \given \bOpE : \type' \times \type'' \rightarrow \type \in \env,
    % % \sig = \interpMap(\bOp{\expr_1'}{\expr_2'}, \worldSet), \\
    % % \qquad \forall \expr_1' \in \texttt{EnumFeatures}(\depth, \env, \type',
    % % \worldSet, ?\expr) \\
    % % \qquad \forall \expr_2' \in \texttt{EnumFeatures}(\depth, \env, \type'',
    % % \worldSet, ?\expr)\}
  % \end{array}\)
\end{minipage}
\caption{Expression Synthesis}
\figlabel{exprSynth}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
\begin{minipage}[htb!]{0.20\textwidth}
\begin{lstlisting}[language=Python, mathescape=true,
xleftmargin=1.0\textwidth,
basicstyle=\scriptsize\ttfamily,
  numbers=left, escapechar=!]
!\(\begin{array}{@{}l}
  \texttt{\textbf{Repair}}
      \nat \times \real \times \worlds \times \worlds \times \pred
      \rightarrow \pred
\end{array}\)!
$\texttt{Repair}$($\minScore$, $\posE$, $\negE$, $\pred$):
  $\texttt{falseNeg} = \texttt{Score}(\pred, \posE, \emptyset) \neq 1.0$ !\label{line:falseNeg}!
  $\texttt{falsePos} = \texttt{Score}(\pred, \negE, \emptyset) \neq 1.0$ !\label{line:falsePos}!
  if ($\texttt{falsePos}$ and $\texttt{falseNeg}$):
    $\pred' = (\pred \land \ppred) \lor (\ppred \land \ppred')$ !\label{line:fullExt}!
  elif ($\texttt{falseNeg}$): $\pred' = \pred \lor \ppred$ !\label{line:orExt}!
  elif ($\texttt{falsePos}$): $\pred' = \pred \land \ppred$ !\label{line:andExt}!
  return ${\arg\max}_{\pred'}~ \texttt{Score}($
    $\texttt{ExprSynth}(\posE, \negE, \pred'), \posE, \negE)$
      $\given \ppred,\ppred' \in \texttt{EnumPredicates}()$ !\label{line:callExpr}!
\end{lstlisting}
\end{minipage}
  \caption{Predicate Repair}
\figlabel{predRepair}
\end{subfigure}
\caption{Predicate Repair Synthesis Algorithms}
\figlabel{dipr_synth}
\end{figure*}


==> language.tex <==

\begin{figure*}[!b]
\scriptsize
\begin{subfigure}{0.65\textwidth}
\lstset{language=model}
\begin{minipage}{0.52\textwidth}
% Operators and Actions
\(
\begin{array}{@{}l@{}c@{\;}l@{\;}l}
\multicolumn{3}{@{}l}{\textbf{Types and Dimensions}} \\
\env  & ::=  & [e:\type]      & \texttt{Type Environment} \\
\dims & ::=  & \dimension{}   & \texttt{Length, Time, Mass}  \\
      & \mid & [0, 0, 0]      & \texttt{Dimensionless} \\
\type & ::=  & \texttt{bool}  & \texttt{Boolean}  \\
      & \mid & \dims          & \texttt{Scalar with dimension \dims} \\
      & \mid & \vect{(\dims)} & \texttt{Vector with \dims-elements} \\[0.4em]
\multicolumn{3}{@{}l}{\textbf{Actions}} \\
\action & ::=  & a & \texttt{Domain-specific action} \\
        & \mid & \startAction & \texttt{Current action} \\
\multicolumn{3}{@{}l}{\textbf{Constant Values}} \\
\thresh & ::= &~\param : \dims & \texttt{Threshold Value} \\
        & \mid & ?\param : \dims & \texttt{Blank Parameter} \\
\end{array}
\)
\end{minipage}
%
~
%
\begin{minipage}{0.4\textwidth}
    % Expressions, Predicates, Policy
    \(\begin{array}{@{}r@{\;}c@{\;}l@{\;}l}
      % Policy
      \multicolumn{4}{@{}l}{\textbf{Action Selection Policy}} \\
      \pol & ::= & \texttt{return}~\action \\
      & \mid &
        \multicolumn{2}{@{}l}{\texttt{if (\pred): $\pol_1$ else $\pol_2$}} \\
      %
      % Predicates
      \multicolumn{4}{@{}l}{\textbf{Predicates}} \\
      \pred & ::=  & \texttt{$\tru$~| $\fls$} \\
      & \mid & \action_1~\texttt{==}~\action_2
      & \hspace{0pt} \\
      & \mid & \expr~\texttt{>}~\thresh \\
      & \mid & \expr~\texttt{<}~\thresh \\
      & \mid & \pred_1~\&\&~\pred_2 \\
      & \mid & \pred_1~||~\pred_2 \\
      & \mid & ?\pred : \texttt{bool} & \texttt{Blank Predicate} \\
      % Expressions
      \multicolumn{4}{@{}l}{\textbf{Expressions}} \\
      \expr & ::=  & \inputVar:\type & \texttt{Input Variable}\\
      & \mid & \const:\type & \texttt{Constant}\\
      & \mid & \multicolumn{2}{l}
      {\hspace{-6pt} \uOp{\expr}} \\
      & \mid & \multicolumn{2}{l}
      {\hspace{-6pt} \bOp{\expr_1}{\expr_2}} \\[.4em]
      & \mid & ?\expr:\type & \texttt{Blank Expression} \\[.4em]
    \end{array}\)
  \end{minipage}

\caption{The language of action selection policies.}
\label{syntax}
\end{subfigure}
~\vrule~
\begin{subfigure}{0.28\textwidth}
\scriptsize
\lstset{language=model}
\begin{minipage}[t!]{0.27\textwidth}
  % Operators and Actions
  \(\begin{array}{@{}c@{\;}c@{\;}l}
    %
    \multicolumn{3}{@{}l}{\textbf{Unary Operators}} \\
    \mathit{op}_1 & ::= &
    \texttt{freePathLength}
    \mid \texttt{angle} \\
    & & \mid \texttt{norm}
    \mid \texttt{abs}
    \mid \texttt{$v_x$}
    \mid \texttt{$v_y$} \\[.4em]
    %
    \multicolumn{3}{@{}l}{\textbf{Binary Operators}} \\
    \mathit{op}_2 & ::= &
    \texttt{angleDist}
    \mid \texttt{dist} \\[.4em]
    %
    \multicolumn{3}{@{}l}{\textbf{Skills}} \\
    \action & ::= &
      \mid \texttt{GoAlone}
      \mid \texttt{Pass} \\
      &  & \mid \texttt{Follow}
      \mid \texttt{Halt} \\[.4em]
    \multicolumn{3}{@{}l}{\textbf{Types and Dimensions for Operations}} \\
    \texttt{abs} & : & \dims \rightarrow  \dims  \\
    \texttt{norm} & : & \vect(\dims) \rightarrow \dims  \\
    \texttt{$v_x$} & : & \vect(\dims) \rightarrow \dims  \\
    \texttt{$v_y$} & : & \vect(\dims) \rightarrow \dims  \\
    \texttt{freePathLength} & : & \vect([1,0,0]) \rightarrow [1, 0, 0]  \\
    \texttt{angle} & : & \vect(\dims) \rightarrow [0,0,0]  \\
    \texttt{angleDist} & : & [0,0,0] \times [0,0,0] \rightarrow [0,0,0]  \\
    \texttt{dist} & : & \vect(\dims) \times \vect(\dims) \rightarrow \dims  \\
  \end{array}\)
\end{minipage}
%
%
  \caption{Social Navigation Domain}
\label{social-domain}
\end{subfigure}

\caption{We write action selection policies in a simple, structured language
(\cref{syntax}). The language it supports several kinds of \emph{blanks}
($?b$, $?x_p$ $?e$), that LDIPS fills in. Every ASP relies on a set of
primtive actions and operators that vary across problem domains.
\cref{social-domain} shows the actions and operators of
Social Navigation ASPs.}
\figlabel{dsl}
\vspace{-2.5em}
\end{figure*}

\section{Synthesis and Repair for Customizable Policy Learning}
%
This section presents a system for learning, customizing, and repairing
robot behaviors as programmatic action selection policies (ASPs).
The robot runs the ASP repeatedly, several times per second,
and uses it to transition between actions, based on the observed state of the
world and the last action taken. Formally, an ASP is a function that maps
a previous action and a current world state to a next action:
$\action \times \world \mapsto \action$.

\subsection{Problem Domains}
% General Introduction to Problem Domains
For generality, \technique{} is agnostic to the problem domain, but requires
specific properties of the domain to be effective.
% What is necessary to define the domain for synthesis?
% Operations
% World State | Input Variables
% Dimensions
% Set of possible Actions
Different problem domains require different sets of primitive actions and
operators for synthesis. We instantiate \technique{} for different
domains by specifying the collection of actions ($\action \in \actions$),
unary operators ($\mathit{op}_1$), binary operators ($\mathit{op}_2$), and
the input variables $(\inputVar$) in the world state ($\world$)
that are relevant to ASPs for that domain.
% Desirable Properties of Domain
% Choices at each step can be separated into actions or "modes"
% The domain uses physical dimensnionality (essentially true for all of robotics)
% Preference is relavent to the domain
% A series of reasonable operations can be used to describe the domain
As such, for a domain to be amenable
to \technique{} it requires that the proceeding components are defined with
the following properties:
\begin{inparaenum}
  \item The relevant decision at each iteration of control can always be reduced
    to an $\action \in \actions$, whether these consist of discrete actions or
    modes of operations.
  \item The operators $\mathit{op}_1$, $\mathit{op}_2$, and
    the world state $\world$ must define the physical dimensions of all
    inputs, outputs, and variables. A domain without varying physical dimensionality
    will see no benefit from \technique{'s} dimensional analysis.
  \item The expressions necessary for critical decision making should be derived
    from some application of
    operators in $\mathit{op}_1$ and $\mathit{op}_2$ to $\inputVar \in \world$.
\end{inparaenum}

% Define the Social Navigation domain
In this work, we evaluate \technique{} by considering the problem of
learning social navigation as an action selection policy (ASP) that
uses low-level actions to direct a robot to reach some goal location efficiently
while safely moving through environments alongside other agents. An ASP for this
task employs four low-level actions to navigate freely (GoAlone),
follow another agent (Follow), pass another agent (Pass), or to come to
a stop (Halt).
These actions and the operators are shown in \cref{social-domain}, and
we define the world state in the reference frame of the robots as
($w = \langle p_g, p_l, p_d, s_d, p_h, v_h, p_{hl}, v_{hl}, p_{hr}, v_{hr} \rangle$)
to be the goal pose ($p_g$), local waypoint position ($p_l$),
the position ($p_d$) and state ($s_d$) of the next door on the navigation path,
and the
positions and velocities of the three closest humans in front of the robot
($p_h, p_{hl}, p_{hr}, v_h, v_{hl}, v_{hr}$).


==> ldips_alg.tex <==
\begin{figure*}[!b]
\begin{minipage}[htb!]{0.33\textwidth}
\begin{lstlisting}[language=Python, mathescape=true,numbers=left,
                   xleftmargin=0.001\textwidth,
                   basicstyle=\scriptsize\ttfamily, escapechar=!]
!\(\begin{array}{@{}l}
  \texttt{\textbf{L1}} :
      \worlds \times \worlds \times \pred \rightarrow \pred
\end{array}\)!
$\texttt{L1}$($\posE$, $\negE$, $\pred$):
  !$\vec{?\param} = \texttt{ParamHoles}(\pred)$!
  !\(\begin{array}{@{}l@{}l@{}l}
    \phi & = & \exists \vec{?\param} \\
    & \mid &
    (\forall \world \in \posE~.~\texttt{PartialEval}(\pred, \world))\land \\
    & &
    (\forall \world \in \negE~.~\neg\texttt{PartialEval}(\pred, \world))
  \end{array}\)!
  return $\texttt{Optimize}$($\phi$)  # $\texttt{MaxSMT}$
!\(\begin{array}{@{}l}
  \texttt{\textbf{ParamHoles}} : \pred \rightarrow [?\param]
\end{array}\)!
!\(\begin{array}{@{}l}
    \texttt{\textbf{PartialEval}} : \pred \times \world \rightarrow \pred
\end{array}\)!
\end{lstlisting}
\end{minipage}
% L2
\begin{minipage}[htb!]{0.38\textwidth}
  \scriptsize
\begin{lstlisting}[language=Python, mathescape=true,
  basicstyle=\scriptsize\ttfamily, numbers=none, numbers=left, escapechar=!]
!\(\begin{array}{@{}l}
  \texttt{\textbf{L2}} :
      \nat \times \env \times \worlds \times \worlds \times \pred
      \rightarrow \pred
\end{array}\)!
$\texttt{L2}$($\depth$, $\env$, $\posE$, $\negE$, $\pred$):
  $\exprs$ = $\texttt{EnumFeatures}$($\maxDepth, \env, \dims, \posE \cup \negE, ?\expr$) !\label{line:enumFeatures}!
  $\pred' = {\arg\max}_{\pred'}~
    \texttt{Score}(\texttt{L1}(\posE, \negE, \pred'), \posE, \negE)$
    $\given \pred' \in \texttt{FillExpressions}(\exprs, \maxDepth)$
  return $\pred'$
!\(\begin{array}{@{}l}
    \texttt{\textbf{FillExpressions}} : \exprs \times \pred \rightarrow \{\pred\}
\end{array}\)!
!\(\begin{array}{@{}l}
    \texttt{\textbf{SigFilter}} : \{ \langle \expr, \sig \rangle \} \rightarrow
                         \{ \langle \expr, \sig \rangle \}
\end{array}\)!
\end{lstlisting}
  % \hrule
  % \vspace{3pt}
  % FillExpressions Def
  \scriptsize
% \end{minipage}
% \vrule
% \hspace{0.5em}
% \begin{minipage}[htb!]{0.45\textwidth}
  \scriptsize
  % \footnotesize
  % enum features
  % \(\begin{array}{@{}l}
    % \texttt{\textbf{EnumFeatures}} :
    % \nat \times \env \times \type \times \worlds \times \expr
    % \rightarrow \{\langle \expr, \sig \rangle\} \\
    % % \texttt{\textbf{Base Case}} \\
    % \texttt{EnumFeatures}(0, \env, \type, \worldSet, \expr) = \{~\} \\
    % % Expansion Rules for hole
    % % \texttt{\textbf{Top-Level Expansion Rule}} \\
    % \texttt{EnumFeatures}(\depth + 1, \env, \type, \worldSet, ?\expr)
    % = \texttt{SigFilter(} \\
    % % Try filling in a constant value
    % % Try filling in an input
    % \quad \{\texttt{EnumFeatures}(\depth, \env, \type, \worldSet, \expr),  \forall \expr : \type \in \env\}~\cup \\
    % % Try applying op1
    % \quad \{\texttt{EnumFeatures}(\depth + 1, \env, \type, \worldSet, \uOp{?\expr}), \\
     % \forall \uOpE : \type' \rightarrow \type \in \env\}) \\
    % % Try Applying op2
    % % \quad \{\texttt{EnumFeatures}(\depth + 1, \env, \type, \worldSet,
    % % \bOp{?\expr}{?\expr}), \\
    % % \qquad  \forall \bOpE : \type' \times \type'' \rightarrow \type \in \env\}) \\
    % % Fundamental constant case
    % % \texttt{\textbf{Fundamental Constant Expansion}} \\
    % \texttt{EnumFeatures}(\depth+1, \env, \type, \worldSet, \const) =
    % \{~\langle \const, \sig \rangle  \\
    % \quad \given \sig = [\const,\dots,\const],
    % \forall \world^i \in \worldSet \}\\
    % % Input Var Case
    % % \texttt{\textbf{Input Variable Expansion}} \\
    % \texttt{EnumFeatures}(\depth+1, \env, \type, \worldSet, \inputVar) =
    % \{~\langle \inputVar, \sig \rangle\ \\
    % \quad \given \sig = [\world^i.\inputVar,\dots,\world^n.\inputVar],
    % \forall \world^i \in \worldSet \} \\
    % % Unary Op Case
    % % \texttt{\textbf{Unary Operator Expansion}} \\
    % \texttt{EnumFeatures}(\depth+1, \env, \type, \worldSet, \uOp{\expr}) =
    % \{~\langle \uOp{\inputVar}, \sig \rangle \\
    % \quad \given \uOpE : \type' \rightarrow \type \in \env,~\sig =
    % [\interp(\uOp{\expr'},\world) \given \world \in \worldSet], \\
    % \qquad\forall \expr' \in
    % \texttt{EnumFeatures}(\depth, \env, \type', \worldSet, ?\expr) \} \\
    % % Binary Op Case
    % % \texttt{\textbf{Binary Operator Expansion}} \\
    % % \texttt{EnumFeatures}(d+1, \env, \type, \worldSet, \bOp{\expr_1}{\expr_2}) =
    % % \{~ \langle \uOp{\inputVar}, \sig \rangle\ \\
    % % \quad  \given \bOpE : \type' \times \type'' \rightarrow \type \in \env,
    % % \sig = \interpMap(\bOp{\expr_1'}{\expr_2'}, \worldSet), \\
    % % \qquad \forall \expr_1' \in \texttt{EnumFeatures}(\depth, \env, \type',
    % % \worldSet, ?\expr) \\
    % % \qquad \forall \expr_2' \in \texttt{EnumFeatures}(\depth, \env, \type'',
    % % \worldSet, ?\expr)\}
  % \end{array}\)
\end{minipage}
% L3
\begin{minipage}[htb!]{0.20\textwidth}
\begin{lstlisting}[language=Python, mathescape=true,
xleftmargin=0.000\textwidth,
basicstyle=\scriptsize\ttfamily,
  numbers=left, escapechar=!]
!\(\begin{array}{@{}l}
  \texttt{\textbf{L3}} :
      \nat \times \env \times \worlds \times \worlds \times \pred
      \rightarrow \pred
\end{array}\)!
$\texttt{L3}$($\depth$, $\env$, $\posE$, $\negE$, $\pred$):
  if ($\texttt{HasPredHoles}(\pred)$):
    $\pred = {\arg\max}_{\pred'}$
      $\texttt{Score}(\texttt{L2}(\maxDepth, \env, \posE, \negE, \pred'), \posE, \negE)$
      $\given \pred' \in \texttt{EnumPredicates}(\maxDepth)$
  if ($\texttt{HasExprHoles}(\pred)$):
    $\pred = \texttt{L2}(\maxDepth, \env, \posE, \negE, \pred)$
  if ($\texttt{HasParamHoles}(\pred)$):
    $\pred = \texttt{L1}(\posE, \negE, \pred)$
  return $\pred$
\end{lstlisting}
\end{minipage}
% \hrule
\caption{LDIPS Algorithms}
\figlabel{LDIPS}
\end{figure*}

